MANAS: Multi-Agent Neural Architecture Search

The Neural Architecture Search (NAS) problem is typically formulated as a graph search problem where the goal is to learn the optimal operations over edges in order to maximise a graph-level global objective. Due to the large architecture parameter space, efficiency is a key bottleneck preventing NAS from its practical use. In this paper, we address the issue by framing NAS as a multi-agent problem where agents control a subset of the network and coordinate to reach optimal architectures. We provide two distinct lightweight implementations, with reduced memory requirements (1/8th of state-of-the-art), and performances above those of much more computationally expensive methods. Theoretically, we demonstrate vanishing regrets of the form O(sqrt(T)), with T being the total number of rounds. Finally, aware that random search is an, often ignored, effective baseline we perform additional experiments on 3 alternative datasets and 2 network configurations, and achieve favourable results in comparison.

==> MANAS Machine Learning Journal/MAformulation.tex <==
\section{Preliminary: Neural Architecture Search}
\label{sec:nasSearch}
%
We consider the NAS problem as formalised in DARTS ~\cite{Liu2019_DARTS}.
At a higher level, the architecture is composed of a \emph{computation cell} that is a building block to be learned and stacked in the network.
The cell is represented by a directed acyclic graph with $V$ nodes and $N$ edges; edges connect all nodes $i,j$ from $i$ to $j$ where $i<j$.
Each vertex $\bm{x}^{(i)}$ is a latent representation 
for $i\in\{1,\ldots,V\}$.
Each directed edge $(i,j)$ (with $i<j$) is associated with an operation $o^{(i,j)}$ that transforms $\bm{x}^{(i)}$.
Intermediate node values are computed based on all of its predecessors as
$
\bm{x}^{(j)} = \sum_{i<j} o^{(i,j)}(\bm{x}^{(i)}).
$
For each edge, an architect needs to intelligently select one operation $o^{(i,j)}$ from a finite set of $K$ operations, $\mathcal{O} = \{o_{k}(\cdot)\}^K_{k=1}$,
where operations represents some function to be applied to $\bm{x}^{(i)}$ to compute $\bm{x}^{(j)}$, e.g., convolutions or pooling layers.
To each $o_{k}^{(i,j)}(\cdot)$ is associated a set of operational weights  $w_{k}^{(i,j)}$ that needs to be learned (e.g. the weights of a convolution filter).
Additionally, a parameter $\alpha_{k}^{(i,j)}\in\mathbb{R}$
characterises the importance of operation $k$ within the pool $\mathcal{O}$ for edge $(i,j)$.
The sets of all the operational weights $\{w_{k}^{(i,j)}\}$ and architecture parameters (edge weights) $\{\alpha_{k}^{(i,j)}\}$ are denoted by $\bm{w}$ and $\bm{\alpha}$, respectively.
DARTS defined the operation $\bar{o}^{(i,j)}(\bm{x})$ as
\begin{equation}\label{eq:darts}
\bar{o}^{(i,j)}(\bm{x})
= \sum_{k=1}^K  \frac{e^{\alpha_{k}^{(i,j)}}}{\sum_{k'=1}^K e^{\alpha_{k'}^{(i,j)}}} \cdot o^{(i,j)}_k(\bm{x})
%\quad\text{for all}\; i,j \in \{1,\dots,V\} \text{ and } i<j
\end{equation}
%
in which $\bm{\alpha}$ encodes the network architecture; and
the optimal choice of architecture is defined by 
%the pair $(\bm{\alpha}^\star,\bm{w}^\star(\bm{\alpha}))$ that solves
%
\begin{align}\label{eq:Optimisation}
\bm{\alpha}^\star = \min_{\bm{\alpha}}
\mathcal{L}^{(\text{val})}( \bm{\alpha},\bm{w}^\star(\bm{\alpha}))
\quad
\text{s.t.}
\quad
\bm{w}^\star(\bm{\alpha}) = \arg\min_{\bm{w}} \mathcal{L}^{( \text{train})}(\bm{\alpha},\bm{w} ).
\end{align}
%where $\bm{w}$ is optimised on the training loss while $\bm{\alpha}$ is optimised on the validation loss.
The  final objective is to obtain a \emph{sparse} architecture $\archi^\star = \{\archi^{(i,j)}\}, 
\forall i,j$ where $\archi^{(i,j)}=[z_{1}^{(i,j)},
\dots,z_{K}^{(i,j)}]$ with $z_{k}^{(i,j)}=1$ for $k$ corresponding to the best operation and $0$ otherwise.
That is, for each pair $(i,j)$ a \emph{single operation} is selected. %Although the final architecture uses exactly one operation per edge, discovering the best operations requires the training of the entire super-network encoded in \eqref{eq:darts}.




\begin{figure}
\centering
\includegraphics[trim={2cm 3cm 5cm 2cm},clip, width = 1\textwidth]{automl4.pdf}
%trim={<left> <lower> <right> <upper>}
\caption{MANAS with single cell. Between each pair of nodes, an agent $\mathcal{A}_i$ selects action $a^{(i)}$ according to $\pi^{(i)}$. Feedback from the validation loss is used to update the policy. %Edges represent operations between two feature maps, and are selected based on individual agents.
}
\label{Fig:MASAUTOML}
\end{figure}



\section{Online Multi-agent Learning for AutoML}
\label{sec:maformu}


NAS suffers from a combinatorial explosion in its search space. A recently proposed approach to tackle this problem is to approximate the discrete optimisation variables (i.e., edges in our case) with continuous counterparts and then use gradient-based optimisation methods.
DARTS~\cite{Liu2019_DARTS} introduced this method for NAS, though it suffers from two important drawbacks. 
First, the algorithm is memory and computationally intensive ($\mathcal{O}(NK)$ with $K$ being total number of operations between a pair of nodes and $N$ the number of nodes) as it requires loading all operation parameters into GPU memory. As a result, DARTS only optimises over a small subset of $8$ repeating cells, which are then stacked together to form a deep network of $20$. Naturally, such an approximation is bound to be sub-optimal.
Second, evaluating an architecture on validation requires the optimal set of network parameters. Learning these, unfortunately, is highly demanding since for an architecture $\mathcal{Z}_{t}$, one would like to compute $\mathcal{L}^{(\text{val})}_{t}\left(\archi_t,\bm{w}^{\star}_{t}\right)$ 
where $\bm{w}^{\star}_{t} = \arg\min_{\bm{w}} \mathcal{L}_{t}^{(\text{train})}(\bm{w}, \mathcal{Z}_{t})$. 
DARTS, uses \emph{weight sharing} that updates $\bm{w}_t$ once per architecture, with the hope of tracking $\bm{w}^{\star}_t$ over learning rounds. Although this technique leads to significant speed up in computation, it is not clear how this approximation affects the validation loss function. 

Next, we detail a novel methodology based on a combination of multi-agent and online learning to tackle the above two problems (Figure~\ref{Fig:MASAUTOML}). Multi-agent learning scales our algorithm, reducing memory consumption by an order of magnitude from $\mathcal{O}(NK)$ to $\mathcal{O}(N)$; and online learning enables rigorous understanding of the effect of tracking $\bm{w}^{\star}_{t}$ over rounds.



\subsection{NAS as a multi-agent problem}


To address the computational complexity we use the weight sharing technique used in DARTS.
However, we handle in a more theoretically grounded way the effect of approximating $\mathcal{L}^{(\text{val})}_{t}\left(\archi_t, \bm{w}^{\star}_{t}\right)$ by  
$\mathcal{L}^{(\text{val})}_{t}\left(\archi_t, \bm{w}_{t}\right)$. 
Indeed, such an approximation can lead to arbitrary bad solutions due to the uncontrollable weight component.
To analyse the learning problem with no stochastic assumptions on the process generating $\nu = \{\mathcal{L}_{1}, \dots, \mathcal{L}_{T}\}$ we adopt an adversarial online learning framework. 


\begin{algorithm}[!ht]
	\begin{algorithmic}[1]
	%\textbf{Input: } ??

\State 	\textbf{Initialize: } $\pi^{i}_1$ is uniform random over all $j\in \{1,\ldots N\}$. And random $\bm{w}_1$ weights.

\State 	\textbf{For} $t=1,\ldots, T$
	
\State 	 $\quad$ {*} Agent $\agent_i$ samples $\bm{a}_{t}^{i} \sim \pi_{t}^{i}(\bm{a}_{t}^{i})$ for all $i\in\{1,\ldots,N\}$, forming architecture $\archi_t$.\label{lst:line:sample}

\State 	 $\quad$ Compute the training loss 
$\loss^{(\text{train})}_t(\bm{a}_t) =\loss^{(\text{train})}_t(\archi_t,\bm{w}_t )$

\State 	 $\quad$ Update $\bm{w}_{t+1}$ for all operation $\bm{a}_{t}^{i}$ in $\archi_t$ from $\bm{w}_{t}$ using back-propagation.

\State 	$\quad$ Compute the validation loss
$\loss^{(\text{val})}_t(\bm{a}_t) =\loss^{(\text{val})}_t(\archi_t,\bm{w}_{t+1} )$ 
	
\State 	 $\quad$ {\textbf{*} Update  $\pi^{i}_{t+1}$} for all $i\in \{1,\ldots N\}$ using $\archi_1,\ldots, \archi_{t}$ and  $\loss^{(\text{val})}_1,\ldots, \loss^{(\text{val})}_{t}$.\label{lst:line:update}
		
\State 	\textbf{Recommend} $\archi_{T+1}$, after round $T$,   where  $\bm{a}_{T+1}^{i} \sim \pi_{T+1}^{i}(\bm{a}_{T+1}^{i})$ for all $i\in\{1,\ldots,N\}$.
	
\caption{
\textsc{General Framework:}
[steps with asterisks (\textbf{*}) are specified in section~\ref{Sec:Sol}]
}
\label{fig:genAl}
\end{algorithmic}
\end{algorithm}



\paragraph{NAS as Multi-Agent Combinatorial Online Learning. }
In Section~\ref{sec:nasSearch}, we defined a NAS problem where one out of $K$ operations needs to be recommended for each pair of nodes $(i,j)$ in a DAG. In this section, we associate \emph{each pair} of nodes with an \emph{agent} in charge of exploring and quantifying the quality of these $K$ operations, to ultimately recommend one.
The only feedback for each agent is the loss that is associated with a global architecture $\archi$, which depends on all agents' choices.

We introduce $N$ decision makers, $\mathcal{A}_{1}, \dots, \mathcal{A}_{N}$ (see Figure~\ref{Fig:MASAUTOML} and Algorithm~\ref{fig:genAl}). 
At training round $t$, each agent chooses an operation (e.g., convolution or pooling filter) according to its local action-distribution (or policy) $\bm{a}_{t}^{j} \sim \pi_{t}^{j}$, for all $j \in \{1, \dots, N\}$ with $\bm{a}_{t}^{j}\in \{1, \dots, K\}$. These operations have corresponding operational weights $\bm{w}_t$ that are learned in parallel. Altogether, these choices $\bm{a}_{t}=\bm{a}_{t}^{1}, \dots, \bm{a}_{t}^{N}$ define a  sparse graph/architecture $\archi_t\equiv \bm{a}_{t}$ for which a validation loss  $\mathcal{L}^{(\text{val})}_{t}\left(\archi_t,\bm{w}_t\right)$ is computed and used by the agents to update their policies. 
%with the goal of approximating an optimal set of policies that minimize cumulative loss.
After $T$ rounds, an architecture is recommended by sampling $\bm{a}_{T+1}^{j} \sim \pi_{T+1}^{j}$, for all $j \in \{1, \dots, N\}$.
These dynamics resemble bandit algorithms where the actions for an agent $\mathcal{A}_{j}$ are viewed as separate arms. 
%In principle, such a strategy can be followed as long as joint exploration between agents is represented. 
This framework leaves open the design of \textbf{1)} the sampling strategy  $\pi^{j}$ and \textbf{2)} how  $\pi^{j}$ is updated from the observed loss.



%\R{ \textsc{Memory efficiency.} One of the main limitations of DARTS is the continuous relaxation which introduces a mixed operation. This is very memory consuming as it requires parameters of all possible operations to be loaded into GPU memory during the search phase. Memory consumption is roughly $N_{\mathcal{O}}$ times larger than in the final model, where $N_{\mathcal{O}}$ represents the number of possible operations (8 in the DARTS implementation). In our approach, we sample a single architecture at each step and hence the memory consumption is the same as in the final model. In DARTS, a cell structure is stacked 8 times during the search phase and then stacked 20 times during the final training of the best architecture due to the memory limitations. In fact, there is no guarantee that the best cell found with 8 stackings is transferable to 20 stackings. Our approach is able to search directly on 20 stackings due to the 1:1 correspondence in memory consumption. This reduced memory consumption also opens up for the possibility to search directly on larger datasets such as ImageNet. The work of \cite{Cai2018_proxylessNAS} also attempts to lower the memory consumption by binarising the mixed operation, although it uses a different search space than DARTS. \textsc{Search space flexibility.} The cell-stacking approach introduces a hard assumption in order to reduce memory requirements. Because we are not limited by this, we learn different operations in each of the stacked cells, as opposed to the learning only two different types of cells as in DARTS.}



% We identify three methodological hurdles  that need to be addressed.


% \textbf{Reducing computational and memory requirement. }
% For architecture $\mathcal{Z}_{t}$ one would like to compute loss $\mathcal{L}^{(\text{val})}_{t}\left(\archi_t,\bm{w}^{\star}_{t}\right)$ 
% where $\bm{w}^{\star}_{t} = \arg\min_{\bm{w}} \mathcal{L}_{t}^{(\text{train})}(\bm{w}, \mathcal{Z}_{t})$. % with $\mathcal{Z}_{t}$ denoting the architecture chosen by the agents at time $t$.
% %not only depends on the actions chosen by agents, but also on additional weight variables (e.g., optimal weights of the neural network) that are typically learned having generated a fixed architecture. In other words, the loss the agents incur depends on both their choices of actions, and on the resultant weight vector of the constructed network, i.e., $\mathcal{L}^{(\text{val})}_{t}\left(\bm{a}_{t}^{(\mathcal{A}_{1})}, \dots, \bm{a}_{t}^{(\mathcal{A}_{N})}, \bm{w}^{\star}_{t}\right)$, where $\bm{w}^{\star}_{t} = \arg\min_{\bm{w}} \mathcal{L}_{t}^{(\text{train})}(\bm{w}, \mathcal{Z}_{t})$ with $\mathcal{Z}_{t}$ denoting the architecture chosen by the agents at time $t$. 
% Unfortunately, this optimization problem easily becomes \textit{computationally} and \textit{memory} intensive, especially when considering deep networks.
% DARTS handles this by updating $\bm{w}_t$ once per step instead of fully training to $\bm{w}^{\star}_t$ each step, an approximation shared by our method.

% In terms of memory load DARTS requires parameters of all possible operations $\bm{\alpha}$ to be loaded into GPU memory during the search phase as a result of the mixed operation in \eqref{eq:darts}.
% Memory consumption is roughly $K$ times larger than in the final model, where $K$ represents the number of possible operations ($K=8$ in the DARTS implementation).
% In contrast, we propose a method that samples \emph{sparse} architectures $\bm{\archi}_t$ with one single operation between nodes at each step and hence the memory consumption is the same as in the final model.
% This offers an improvement of the memory load over DARTS by a factor equal to the number of available operations $K$.

% In DARTS, a computational cell is stacked $8$ times during search and then $20$ times during the final training of the best architecture due to memory restrictions---which is bound to be sub-optimal. 
% Thanks to the 1:1 correspondence in memory consumption in search and augmentation phases, we are able to search directly on $20$ stackings, which opens up the possibility to search directly on larger datasets such as ImageNet.
% The cell-stacking approach introduces a hard assumption in order to reduce memory requirements.
% Because we are not limited by this, we learn different operations in each of the stacked cells, as opposed to the learning only two different types of cells as in DARTS.


%This will ultimately reduce the memory load to its bare minimum in the back-propagation step to update $w_t$ as less operations will be active. Moreover the sampling technique will directly be in charge of choosing $\archi_t$.
%We limit ourself to sampling \emph{sparse} architectures $\bm{\archi}$, with one single operation between nodes, at each round $t$ in order to achieve \emph{memory-optimality}. 
%Therefore our method combines the computational lightness (using $w_t$) and memory lightness (sparse architecture).


%\todo{can we really say that we solve for $w^\star$ its more a gradient descent on both $w^\star$ and $\alpha$ at the same time, and the problem is that all the operation are active}

%\textbf{Addressing  uncontrollable operational weights $\bm{w}_t$ with adversarial regret. } 
%Computing 
%$\mathcal{L}^{(\text{val})}_{t}\left(\archi_t, \bm{w}_{t}\right)$ 
%$\mathcal{L}^{(\text{val})}_{t}\left(\bm{a}_{t}^{(\mathcal{A}_{1})}, \dots, \bm{a}_{t}^{(\mathcal{A}_{N})}, \bm{w}_{t}\right)$ 
%instead of 
%$\mathcal{L}^{(\text{val})}_{t}\left(\archi_t, \bm{w}^{\star}_{t}\right)$
%$\mathcal{L}^{(\text{val})}_{t}\left(\bm{a}_{t}^{(\mathcal{A}_{1})}, \dots, \bm{a}_{t}^{(\mathcal{A}_{N})}, \bm{w}^{\star}_{t}\right)$
%can lead to arbitrary bad solutions due to the uncontrollable weight component.
%This motivates us to design \emph{theoretically grounded} methods that are able to learn with \emph{arbitrary} data where no stochastic assumptions are made on the process generating $\nu = \{\mathcal{L}_{1}, \dots, \mathcal{L}_{T}\}$. %\todo{are we talking about the methods that we will provide in the next section?}
%Unfortunately, computing a solution to such a bi-level optimisation problem easily becomes computationally and memory intensive, especially when considering deep networks as function approximators. DARTS, for instance, handled such a complexity exhaustively, by solving for $\bm{w}^{\star}$ at each iteration of the algorithm. Rather than following a similar expensive technique, we advocate a more \emph{memory-optimal} which descends one step per-each round. 
%Although optimal in memory, the above solution introduces additional randomness to the loss function (due to the uncontrollable weight component), which if not considered, leads to arbitrary bad solutions. Consequently, algorithms that only minimise standard regret forms (e.g., performance against the best in hind-sight) is not ideal for efficient neural architecture search. \todo{are we talking about the methods that we will provide in the next section?}
%\todo{emphasize the use of sparse architecture for memory saving?}
%
%The problem when agents receive arbitrary losses for their action selections has been well-studied 
%However, we still expect some operations to perform overall better than others over time, therefore, our algorithms can be analyzed  as in online learning under adversarial bandit settings: 

%Given $\nu$,  minimise worst-case regret under any loss observation.  We now introduce two notions of regret that motivates our proposed approaches.

\paragraph{Minimization of worst-case regret under any loss. }
The following two notions of regret motivate our proposed NAS method.
Given a policy $\pi$ the  \emph{cumulative regret} $\mathcal{R}_{T,\pi}^{\star} $ and the  \emph{simple regret} $ r_{T,\pi}^{\star}$ after $T$ rounds and under the worst possible environment $\nu$,  are:
% \begin{align}
%     \mathcal{R}_{T}^{\star}(\pi) &= \sup_{\nu}  \mathbb{E}\left[\sum_{t=1}^{T} \mathcal{L}_{t}(\bm{a}_{t}) - \min_{\bm{a}}\sum_{t=1}^{T}\mathcal{L}_{t}(\bm{a})\right], \label{cregret_def} 
%       r_{T}^{\star}(\pi) =  \sup_{\nu} \mathbb{E}\left[\sum_{t=1}^{T} \mathcal{L}_{t}(\bm{a}_{T+1}) - \min_{\bm{a}}\sum_{t=1}^{T}\mathcal{L}_{t}(\bm{a})\right],\label{sregret_def}
% \end{align}
\begin{align}\label{cregret_def} 
    \mathcal{R}_{T,\pi}^{\star} &= \sup_{\nu}  \mathbb{E}\sum_{t=1}^{T} \mathcal{L}_{t}(\bm{a}_{t}) - \min_{\bm{a}}\sum_{t=1}^{T}\mathcal{L}_{t}(\bm{a}),\\
    \label{sregret_def} 
      r_{T,\pi}^{\star} &=  \sup_{\nu} \mathbb{E}\sum_{t=1}^{T} \mathcal{L}_{t}(\bm{a}_{T+1}) - \min_{\bm{a}}\sum_{t=1}^{T}\mathcal{L}_{t}(\bm{a})
\end{align}
where the expectation is taken over both the losses and policy distributions, and $\bm{a} = \{\bm{a}^{(\mathcal{A}_j)}\}^{N}_{j=1}$ denotes a joint action profile. 
The simple regret leads to minimising the loss of the recommended architecture $a_{T+1}$, while minimising the cumulative regret adds the extra requirement of having to sample, at any time $t$, architectures with close-to-optimal losses. We  discuss in the appendix~\ref{sec:discussion} how this requirement could improve in practice the tracking of $\bm{w}_t^\star$ by $\bm{w}_t$.
We let $\mathcal{L}_{t}(\bm{a}_{t})$ be potentially adversarilly designed to account for the difference between $\bm{w}_t^\star$ and $\bm{w}_t$ and make no assumption on its convergence. Our models and solutions in Section~\ref{Sec:Sol} are designed to be robust to arbitrary $\mathcal{L}_{t}(\bm{a}_{t})$.
%Minimising expected regret, however, does not suffice for well-behaving algorithms due to the arbitrary nature of the received losses. For this reason, adversarial bandits seek algorithms that minimise worst-case regret (i.e., regret under worst-case environments), defined as: 
%\begin{equation*}
%    \mathcal{R}_{T}^{\star}(\pi) = \sup_{\nu} \mathcal{R}_{T}(\pi, \nu), \quad\text{and}\quad r_{T}^{\star}(\pi) = \sup_{\nu} r_{T}(\pi, \nu).
%\end{equation*}

Because of the discrete nature of the NAS problem, during search the loss can take on large values or alternate between large and small values arbitrarily. Gradient-descent methods perform best under smooth loss functions, which is not the case in NAS.
The worst-case regret minimization is a theoretically-grounded objective which we make use of in order to provide guarantees on the convergence of the algorithm when no assumptions are made on the process generating the losses.

\section{Adversarial Implementations}\label{Sec:Sol}
%This section elaborates our solution methods for neural architecture search when considering adversarial weight updates. We propose two algorithms that implicitly enable coordination between agents through shared loss functions. Our first algorithm, achieves credit-assignment through approximating validation losses as linear combinations of edge weights, thus, implicitly, achieving multi-agent credit assignment and discuss sampling techniques that aim at minimizing either the cumulative or simple regret. Though successful, linear approximations to deep network validation losses can easily become crude. Therefore, we extend our approach to support non-linear losses as discussed in Section~\ref{Sec:ACO}.
%
In the following subsections we will describe our proposed approaches for NAS when considering adversarial losses. We present two algorithms, MANAS and MANAS-LS, that implement two different \emph{credit assignment techniques}  specifying the update rule in line~\ref{lst:line:update} of Algorithm~\ref{fig:genAl}.
The first  approximates the validation loss as a linear combination of edge weights, while the second handles non-linear losses.

Note that \textit{adversarial} in this context refers to the adversarial multi-arm bandit \cite{auer1995gambling} framework: we  model the fact that a weight-sharing supernetwork returns noisy rewards as having an adversary that explicitly tries to confuse the learner.
Adversarial multi-arm bandit is the strongest generalization of the bandit problem, as it removes all assumptions on the distribution.
Our MA formulation and algorithm explicitly account for this adversarial nature and provide a principled solution that is provably robust.
%a solution to the adversarial bandit problem is a generalized solution to the more specific bandit problems.
%We propose two associated sampling techniques that specify line~\ref{lst:line:sample} of Algorithm~\ref{fig:genAl}, one minimising the \emph{cumulative regret}  (\ref{cregret_def}), and one targeting the \emph{simple regret} (\ref{sregret_def}).


%Our solution is to introduce approximate credit assignments that quantify the effect of actions chosen with respect to the overall validation loss. This allows the agents to coordinate implicitly and remedy the combinatorial explosion.
%introducing two sets of algorithms for neural architecture search using online multi-agent learning. 
%
%We  remedy the combinatorial explosion in the possible number of paths by considering coordination between agents. Moreover, we deal with the losses by introducing an approximate credit assignment between agents that quantifies the effect of actions chosen with respect to the overall validation loss. \todo{} 
%%
% Unfortunately, adversarial regret frameworks described above are inapplicable in our scenario for several reasons. First of all, most algorithms with vanishing adversarial regret assume a single-agent and linear loss setting. Clearly, our problem introduces multiple agents in need of co-ordination for successful behaviour, and losses are nonlinear due to our focus on deep neural networks.\footnote{Also notice that in our scenario, the agent has an indirect role in the loss due to the execution of one gradient step. We believe better algorithms can be attained by exploiting this fact. We leave such a study for future work.}. Second of all, when defined naively, our problem is combinatorial due the explosion in the total number of possible paths going from initial to final nodes. Third, our approach is less concerned with cumulative regret but rather with the minimum loss value acquired over round. 
%
% In what comes next, we remedy the above problems by introducing two algorithms for neural architecture search using online multi-agent learning. We redefine the notion of regret to better suit neural architecture search problems, and remedy the combinatorial explosion in the possible number of paths by considering coordination between agents. Moreover, we deal with nonlinear losses by introducing an approximate credit assignment between agents that quantifies the effect of actions chosen with respect to the overall validation loss.
%
%\paragraph{Decomposition of the loss by approximate credit assignment}\label{ssec:Decomposition}
%\subsection{\textcolor{autored}{Decomposition of the Loss: Approximating Credit-Assignment}}\label{ssec:Decomposition}
% Though reducing the size of the search space, the simplification of independent learners induces additional communication complexity, where agents now need to coordinate to acquire a solution. 




\subsection{MANAS-LS}

\paragraph{Linear Decomposition of the Loss. }
A simple credit assignment strategy is to approximate edge-importance (or edge-weight) by a vector $\bm{\beta}_{s}\in\mathbb{R}^{KN}$ representing the importance of all $K$ operations for each of the $N$ agents. 
$\bm{\beta}_{s}$ is an arbitrary, potentially adversarially-chosen vector and varies with time $s$ to account for the fact that the operational weights $\bm{w}_{s}$ are learned online and to avoid any restrictive assumption on their convergence.
The relation between the observed loss $\mathcal{L}_{s}^{(\text{val})}$ and the architecture selected at each sampling stage $s$ is modeled through a linear combination of the architecture's edges (agents' actions) as
%Even against such adversity, agents can still reason about the environment for well-behaved algorithms, if they are capable of measuring their action effect on the $t^{th}$ validation loss. In multi-agent literature, this problem is typically referred to as multi-agent credit-assignment one. Please notice that in AutoML, this problem amounts to understanding the effect of an operation on the resulting overall loss. Clearly, seeking a closed form analytical solution to this problem is challenging. As such, we follow an simplified approximation scheme, shown effective in experiments, see Section~\ref{sec:exp}, to assign credit to each of the agents' action choices. Precisely, we attempt to approximate edge-importance (or edge-weight) through a linear combination of the architecture's edges (i.e., agents' actions). Namely, we assume that the validation loss can be written as:
\begin{equation}
    \mathcal{L}_{s}^{(\text{val})} 
    = \bm{\beta}_{s}^{\mathsf{T}} \bm{Z}_{s}
\end{equation}
where $\bm{Z}_{s}\in\{0,1\}^{KN}$ is a vectorised one-hot encoding of the architecture $\mathcal{Z}_{s}$ (active edges are 1, otherwise 0).
%Every time we sample an architecture $\bm{Z}_{s}$ and compute its validation accuracy $\mathcal{L}_{s}^{(\text{val})}$, we obtain a row of a system of linear equations $\mathcal{L}^{(\text{val})} = \bm{\beta}_t^{\mathsf{T}} \bm{Z}$. 
After evaluating $S$ architectures, at round $t$ we estimate $\bm{\beta}$ by solving the following via least-squares: 
\begin{equation}
\text{Credit assignment:~~~}
\bm{ \widetilde B}_{t} = \text{arg}\min_{\bm{\beta}} 
\sum_{s=1}^{S} 
\left(\mathcal{L}_{s}^{(\text{val})} - \bm{\beta}^{\mathsf{T}}  \bm{Z}_{s}\right)^{2}.
\end{equation}
%
The solution gives an efficient way for agents to update their corresponding action-selection rules  and leads to implicit coordination. 
Indeed, in Appendix~\ref{app:facReg} we demonstrate that the worst-case regret $\mathcal{R}^\star_{T}$~(\ref{cregret_def})  can actually be decomposed into an agent-specific form $\mathcal{R}^{i}_T\left(\boldsymbol{\pi}^{i},\nu^{i}\right)$ defined in the appendix:
$
    \mathcal{R}^\star_{T} = \sup_{\nu}\mathcal{R}_{T}(\bm{\pi}, \nu) \iff   \sup_{\nu^{i}}\mathcal{R}^{i}_T\left(\boldsymbol{\pi}^{i},\nu^{i}\right), \ \ \ i=1,\ldots,N$.
This decomposition allows us to significantly reduce the search space complexity by letting each agent $\mathcal{A}_i$ determine the best operation for the corresponding graph edge.

%and apply upcoming sampling techniques for each agent $\mathcal{A}_i$ in a completely parallel fashion.


\paragraph{Zipf Sampling for $r_{T,\pi}^{\star}$. }
$\mathcal{A}_i$ samples an operation $k$ proportionally to the inverse of its estimated rank $\widetilde{ \langle k \rangle }^{i}_t$, where $\widetilde{ \langle k \rangle }^{i}_t$ is computed by sorting the operations
of agent $\mathcal{A}_i$ w.r.t $\tilde{\boldsymbol{B}}^{i}_t[k] $, as
%
\[
%P\left(\bm{a}_{t}^{(i)}=k\right)
 \text{Sampling policy:~~~}
\boldsymbol{\pi}^{i}_{t+1}[k] 
 %= \frac{1}{\widetilde{ \langle k \rangle }^{(\mathcal{A}_i)}_t\overline{\log K}} \quad \text{ where } \overline{\log K} = \sum_{k=1}^K\frac{1}{k}.
  = 1
  \Big/
  \widetilde{ \langle k \rangle }^{i}_t\overline{\log} K \quad \text{ where } \overline{\log} K = 1+1/2+\ldots+1/K.
\]
%
Zipf explores efficiently, 
%as, up to log factors,  for  $1\leq m \leq K$,  the $m$  estimated best operations  are picked uniformly ignoring the remaining $K-m$ operations.% All operations are explored almost as in uniform exploration while the estimated best  is picked almost all the time.
%The Zipf law 
is anytime, parameter free, minimises optimally the simple regret in   multi-armed bandits when the losses are adversarially designed and adapts optimally to stationary losses~\cite{abbasi2018best}.


We prove for this new algorithm an exponentially decreasing simple regret $r^\star_{T}= \mathcal{O}\left(e^{-T/H}\right)$, where $H$ is a measure of the complexity for discriminating sub-optimal solutions as $H=N(\min_{j\neq k^\star_i,1\leq i \leq N\} }\boldsymbol{B}^{i}_T[j]-\boldsymbol{B}^{i}_T[k^\star_i] )$, where $k^\star_i= \min_{1\leq j \leq K }\boldsymbol{B}^{i}_T[j])$ and $\boldsymbol{B}^{i}_T[j]=\sum_{t=1}^T \boldsymbol{\beta}^{(\mathcal{A}_i)}_t[j]$. 
%This results from using special unbiased estimates of $\boldsymbol{B}^{(\mathcal{A}_i)}_T[j]$ and having a sampling strategy that samples all operations with positive probability.
The proof in given in Appendix~\ref{app:theoryLZ}.


\subsection{MANAS}

\paragraph{Coordinated Descent for Non-Linear Losses. }
\label{Sec:ACO}
%
In some cases the linear approximation may be crude.
An alternative is to make no assumptions on the loss function and have each agent directly associate the quality of their actions with the loss $\loss^{(\text{val})}_t(\bm{a}_t) $.
%we propose now an alternative approach where
%each agent consider the other agents as part of the adversarial environment (this contradicts coordination, doesn't it?) and optimize its own choice and loss ignoring the actions performed by the other agents.
This results in all the agents performing a coordinated descent approach to the problem. Each agent updates for operation $k$ its $\bm{ \widetilde B}^{i}_{t}[k]$ as
%
\begin{equation}
 %\text{Update:~~~}\bm{ \widetilde B}^{(\mathcal{A}_i)}_{t}[k] = \bm{ \widetilde B}^{(\mathcal{A}_i)}_{t-1}[k]+ \frac{\loss^{(\text{val})}_t(\bm{a}^{(\mathcal{A}_1)}_t,\ldots, \bm{a}^{(\mathcal{A}_N)}_t) \mathbbm{1}_{ \bm{a}_{t}^{(\mathcal{A}_i)} = k }}{\boldsymbol{\pi}^{(\mathcal{A}_i)}_t[k]}.
\text{Credit assignment:~~}
\bm{ \widetilde B}^{i}_{t}[k] = \bm{ \widetilde B}^{i}_{t-1}[k]+ \loss^{(\text{val})}_t \cdot \mathbbm{1}_{ \bm{a}_{t}^{i} = k }/\boldsymbol{\pi}^{i}_t[k].
\label{eq:MANAS_credit}
\end{equation}


\paragraph{Softmax Sampling for $\mathcal{R}_{T,\pi}^{\star}$. }
Following EXP3~\cite{auer2002nonstochastic}, %and Hedge~\cite{freund1997decision} algorithms
actions are sampled from a softmax distribution (with temperature $\eta$) w.r.t.  $\tilde{ \boldsymbol{B}}^{i}_t[k]$:
%and the aim is to always choose the best operation given the following softmax distribution ($k \in \{1,\dots,K\}$):
 %
\[
 \text{Sampling policy:~~}
 %\boldsymbol{\pi}^{(\mathcal{A}_i)}_{t+1}[k] = \frac{\exp\left(\eta\boldsymbol{\tilde B}^{(\mathcal{A}_i)}_t[k] \right)}{\sum_{j=1}^{K}\exp\left(\eta\boldsymbol{\tilde B}^{(\mathcal{A}_i)}_t[j] \right)} \text{ for }k = 1,\ldots,K.
 \boldsymbol{\pi}^{i}_{t+1}[k] = \exp\left(\eta 
 \tilde{\boldsymbol{B}}^{i}_t[k] \right)
 \Big/
 \sum_{j=1}^{K}\exp\left(\eta \tilde{\boldsymbol{B}}^{i}_t[j] \right).
 \]
%
Using this sampling strategy, EXP3 \cite{auer2002nonstochastic} is run for each agent in parallel. If the regret of each agent is computed by considering the rest of the agent as fixed, then each agent has regret $\mathcal{O}\left(\sqrt{TK\log K}\right)$ which sums over agents to $\mathcal{O}\left(N\sqrt{TK\log K}\right)$.
The proof is given in Appendix \ref{app:theoryLZ}



\paragraph{On credit assignment.}
Our MA formulation provides a gradient-free, credit assignment strategy. Gradient methods are more susceptible to bad initialisation and can get trapped in local minima more easily than our approach, which, not only explores more widely the search space, but makes this search optimally according to multi-armed bandit derived regret minimization. 
Concretely, MANAS can easily escape from local minima as the reward is scaled by the probability of selecting an action (Eq.~\ref{eq:MANAS_credit}). Thus, the algorithm has a higher chance of revising its estimate of the quality of a solution based on new evidence. This is important as one-shot methods (such as MANAS and DARTS) change the network---and thus the environment---throughout the search process. Put differently, MANAS' optimal exploration-exploitation allows the algorithm to move away from 
`good' solutions towards `very good' solutions that do not live in the former's proximity; in contrast, gradient methods will tend to stay in the vicinity of a `good' discovered solution.

==> MANAS Machine Learning Journal/discussion.tex <==
\section{Discussion}
\label{sec:discussion}


\paragraph{Random Baselines.}
Clearly, in specific settings, random sampling performs very competitively. On one hand, since the search space is very large (between $8^{112}$ and $8^{280}$ architectures exist in the DARTS experiments), finding the global optimum is practically impossible. %that outperforms a random baseline.
Why is it then that the randomly sampled architectures are able to deliver nearly state-of-the-art results?
Previous experiments \cite{Sciuto2019_random,Li2019_random} together with the results presented here seem to indicate that the available operations and meta-structure have been carefully chosen and, as a consequence, most architectures in this space generate very good results.
This suggests that human effort has simply transitioned from finding a good architecture to finding a good search space---a problem that needs careful consideration in future work. 
Random search with WS \cite{Li2019_random}, has also shown to perform competitively but it is clearly sub-optimal compared to our multi-agent framework.

\paragraph{On fair evaluation. }
It is worth stressing that we performed all comparisons using the same final training protocol. This is extremely relevant as there has been a recent trend to boost results simply by stacking more training tricks on to the evaluation protocol.
As such, any improvement in the final accuracy is solely due to how the network was trained rather than the quality of the search method used or the architecture discovered \cite{Yang2020NASEFH}. 

\paragraph{Agent coordination, combinatorial explosion and approximate credit assignment. }
%\textbf{Combinatorial explosion and coordination of agents through credit assignment. } 
%Unfortunately, we need to be careful when applying the adversarial regret frameworks described above. 
%First of all, most algorithms with vanishing adversarial regret assume a single-agent and linear loss setting.
Our set-up introduces multiple agents in need of coordination.
%, and losses are intricate functions of each agent choices due to our focus on deep neural networks.
%\footnote{Also notice that in our scenario, the agent has an indirect role in the loss due to the execution of one gradient step. We believe better algorithms can be attained by exploiting this fact. We leave such a study for future work.}
%Moreover, 
Centralised critics use explicit coordination and learn the value of coordinated actions across all agents~\cite{Shimon}, but the complexity of the problem grows exponentially with the number of possible architectures $\archi$, which equals $K^N$.
%However, the requirement for centralized information severely limits this approach's scalability.
We argue instead for an implicit approach where coordination is achieved through a joint loss function depending on the actions of all agents. This approach is scalable as each agent searches its local action space---small and finite---for optimal action-selection rules.
Both credit assignment methods proposed learn, for each operation $k$ belonging to an agent $\mathcal{A}_{i}$, a quantity $\bm{ \widetilde B}^{i}_{t}[k] $ (similar to $\alpha$ in Section \ref{sec:nasSearch}) that quantifies the contribution of the operation to the observed losses.

==> MANAS Machine Learning Journal/experiments.tex <==
\begin{comment}

\begin{table}[t]
  \caption{Comparison with state-of-the-art image classifiers on ImageNet (mobile setting) }
  \label{table:ImageNetresults}
  \centering
  \begin{tabular}{p{6cm}p{1.5cm}p{1cm}p{1.8cm}p{1.5cm}llllllll}
    \toprule
    \cmidrule(r){1-2}
    Architecture   & Test Error (\%) & Params (M) & Search Cost (GPU days) & Search Method\\
    \midrule
    %Inception-v1 \cite{Szegedy2017_inception} & $30.2$ & $6.6$ & & manual \\
    %MobileNet \cite{Howard2017_MobileNets} & $29.4$ & $4.2$ & & manual \\
    %ShuffleNet 2x (v1) \cite{Ma2018_ShuffleNetV1} & $29.1$ & ~$5$ & & manual \\
    ShuffleNet 2x (v2)  \cite{Zhang2018_ShuffleNetV2} & $26.3$ & ~$5$ & & manual \\
    \midrule
    NASNet-A \cite{Zoph2018_NASNet} & $26.0$ & $5.3$ & $1800$ & RL \\
    %NASNet-B \cite{Zoph2018_NASNet} & $27.2$ & $5.3$ & $1800$ & RL \\
    %NASNet-C \cite{Zoph2018_NASNet} & $27.5$ & $4.9$ & $1800$ & RL \\
    %AmoebaNet-A \cite{Real2018_AmoebaNet} & $25.5$ & $5.1$ & $3150$ & evolution \\
    %AmoebaNet-B \cite{Real2018_AmoebaNet} & $26.0$ & $5.3$ & $3150$ & evolution \\
    AmoebatNet-C \cite{Real2018_AmoebaNet} & $24.3$ & $6.4$ & $3150$ & evolution \\
    PNAS \cite{Liu2018_PNAS} & $25.8$ & $5.1$ & ~$225$ & SMBO \\
    SNAS \cite{Xie19_SNAS} & $27.3$ & $4.3$ & $1.5$ & gradient \\
    DARTS \cite{Liu2019_DARTS} & $26.7$ & $4.7$ & $4$ & gradient      \\
    \midrule
    Random sampling & $27.75$ & $2.5$ & --- & --- \\ 
    \our (searched on CIFAR-10) & $26.47$ & $2.6$ & $2.8$ & MA \\ 
    \our (searched on CIFAR-10) + AA & \Blue{????} & $2.6$ & $2.8$ & MA \\ 
    \our (searched on ImageNet) & $26.15$ & $2.6$ & $110$ & MA \\
    \our (searched on ImageNet) + AA & \Blue{????} & $2.6$ & $110$ & MA \\
    \bottomrule
  \end{tabular}
\end{table}

\end{comment}


We (1) compare \our against existing NAS methods on the well established CIFAR-10 dataset; (2) evaluate \our on ImageNet; (3) compare \our, DARTS, Random Sampling and Random Search with WS \cite{Li2019_random} on $3$ new datasets (Sport-8, Caltech-101, MIT-67); and (4) evaluate \our with inference time as complexity constraint.
Descriptions of the datasets and details of the search are provided in the Appendix.
% \cite{Krizhevsky2009_cifar,Deng2009_imagenet,li2007_sport8,fei2007_caltech101,quattoni2009_mit67}
We report the performance of two algorithms, \our and \our-LS, as described in Section~\ref{Sec:Sol}. 
Note that, with the exception of results marked as \textit{+AutoAugment}, all experiments were run with the same final training protocol as DARTS \cite{Liu2019_DARTS}, for fair comparison.
%Linear+Softmax proved in preliminary experiments to be harder to tune and was thus excluded from further experiments.
%Linear+Softmax gave similar results with more hyperparameters to tune (Boltzmann temperature) and was thus excluded from further experiments.

\paragraph{Search Spaces.} 
We use the same CNN search space as \cite{Liu2019_DARTS}. Since \our is memory efficient, it can search for the final architecture without needing to stack \textit{a posteriori} repeated cells; thus, all our cells are unique.
For fair comparison, we use $20$ cells on CIFAR-10 and $14$ on ImageNet.
Experiments on Sport-8, Caltech-101 and MIT-67 in Section~\ref{sec:alt_expers} use both $8$ and $14$ cell networks.

\paragraph{Search Protocols.}
For datasets other than ImageNet, we use $500$ epochs during the search phase for architectures with $20$ cells, $400$ epochs for $14$ cells, and $50$ epochs for $8$ cells.
All other hyperparameters are as in \cite{Liu2019_DARTS}.
For ImageNet, we use $14$ cells and $100$ epochs during search.
In our experiments on the three new datasets we rerun the DARTS code to optimise an $8$ cell architecture; for $14$ cells we simply stacked the best cells for the appropriate number of times.



\paragraph{Synthetic experiment.}
To illustrate the theoretical properties of MANAS we apply it to the Gaussian Squeeze task, a problem where agents must coordinate their actions in order to optimize a global objective function that depends on the actions of each agent \cite{yang2018mean,colby2015}.
Specifically, $N$ homogeneous agents determine their individual actions $a^{(j)}$ to jointly optimize the objective 
$G(x) = x e^{-\frac{(x-\mu)^{2}}{\sigma^{2}}}$
where $x = \sum_{j=1}^{N} a^{(j)}$.
This synthetic setup has the same characteristics of the multi-agent NAS problem, namely a group of agents \textit{implicitly} coordinating their actions to achieve a global objective, and is therefore a good experiment to showcase the theoretical properties of the MANAS algorithm.

We confirm that (1) MANAS progresses steadily towards zero regret while the Random Search baseline struggles to move beyond the initial starting poin; (2) MANAS stays well within the theoretical cumulative regret bound (Figure~\ref{fig:gsd}).

\begin{figure}[!h]
\centering
\includegraphics[width=0.5\textwidth]{MANAS_GaussianSqueezeDomain.pdf}%
%\caption{Regret for the Gaussian Squeeze Domain experiment with $100$ agents, $10$ actions, $\mu=1$, $\sigma=10$.}
%\label{fig:gsd}
\includegraphics[width=0.5\textwidth]{MANAS_GaussianSqueezeDomain_theoryBound.pdf}%
\caption{
Left: Regret for the Gaussian Squeeze Domain experiment with $100$ agents, $10$ actions, $\mu=1$, $\sigma=10$.
Right: Theoretical bound for the MANAS cumulative regret ($2N\sqrt{TK\log K}$; see Appendix~\ref{app:theoryCS}) and the observed counterpart for the Gaussian Squeeze Domain experiment with $100$ agents, $10$ actions, $\mu=1$, $\sigma=10$.
}
\label{fig:gsd}
\end{figure}



\begin{table}[t]
  \caption{Comparison with state-of-the-art image classifiers on CIFAR-10. The four row blocks represent: human-designed, NAS, MANAS search with DARTS training protocol and best searched MANAS retrained with extended protocol (AutoAugment + 1500 Epochs + 50 Channels). Unless specified, all architectures use 20 cells.}
  \label{table:Cifarresults}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{p{5.3cm}p{1.5cm}p{1cm}p{1.8cm}p{2.0cm}}
    \toprule
    %\cmidrule(r){1-2}
    Architecture   & Test Error ($\%$)     & Params (M) & Search Cost (GPU days) & Search Method\\
    \midrule
    DenseNet-BC \cite{Huang2017_densenet} & $3.46$ & $25.6$ & --- & manual \\
    \midrule
    NASNet-A \cite{Zoph2018_NASNet} & $2.65$ & $3.3$ & $1800$ & RL \\
    %AmoebaNet-A \cite{Real2018_AmoebaNet} & $3.34$ & $3.2$ & $3150$ & evolution \\
    AmoebaNet-B \cite{Real2018_AmoebaNet} & $2.55$ & $2.8$ & $3150$ & evolution \\
    %Hierarchical Evo \cite{Liu18_HEVO} & $3.75$ & $15.7$ & $300$ & evolution \\
    PNAS \cite{Liu2018_PNAS} & $3.41$ & $3.2$ & $225$ & SMBO \\
    ENAS \cite{Pham2018_ENAS} & $2.89$     & $4.6$ & $0.5$ & RL \\
    SNAS \cite{Xie19_SNAS} & $2.85$ & $2.8$ & $1.5$ & gradient \\
    DARTS, 1st order \cite{Liu2019_DARTS} & $3.00$ & $3.3$ & $1.5^{\dagger}$ & gradient     \\
    DARTS, 2nd order \cite{Liu2019_DARTS} & $2.76$ & $3.3$ & $4^{\dagger}$ & gradient      \\
    %GHN \cite{DBLP:conf/iclr/ZhangRU19} & $2.84$ & $5.7$ & $0.84$ & RS+WS      \\
    SDARTS-ADV \cite{DBLP:conf/icml/ChenH20} & $2.61$ & $3.3$ & $4.3$ & gradient      \\
    DARTS- \cite{DBLP:conf/iclr/ChuW0LWY21} & $2.63$ & $3.5$ & $4^{\dagger}$ & gradient      \\
    GDAS\cite{DBLP:conf/cvpr/DongY19} & $3.75$ & $3.4$ & $0.17$ & gradient      \\
    NPENAS-BO\cite{wei2022npenas} & $2.52$ & $4.0$ & $2.5$ & evolution      \\
    EffPNet\cite{wang2021surrogate} & $3.49$ & $2.54$ & $3$ & evolution \\ 
    BANANAS\cite{white2021bananas} & $2.64$ & $-$ & $11.8$ & BO + predictor \\ 
    %P-DARTS + cutout & 2.50 & 3.4 & 0.3 & gradient \\
    Random + cutout \cite{Liu2019_DARTS} & $3.29$ & $3.2$ & --- & --- \\
    Random Search WS \cite{Li2019_random} & $2.85$  & $4.3$ & $9.7$ & random search\\
    \midrule
    \our (8 cells) & $3.05$ & $1.6$ & $0.8^{\dagger}$ & MA\\
    \our & $2.63$ & $3.4$ & $2.8^{\dagger}$ & MA \\
    \our--LS  & $\bm{2.52}$ & $3.4$ & $4^{\dagger}$ & MA \\ 
    \midrule
    \our + AutoAugment & 1.97 & $3.4$ & --- & MA \\ 
    \our--LS  + AutoAugment & 1.85 & $3.4$ & --- & MA \\ 
    \bottomrule
    \multicolumn{5}{p{\dimexpr\textwidth-2\tabcolsep\relax}}{$^{\dagger}$ {\small Search cost is for $4$ runs and test error is for the best result (for a fair comparison with other methods).}}
  \end{tabular}
  }
\end{table}



\subsection{Results on CIFAR-10}

\paragraph{Evaluation.}
To evaluate our NAS algorithm, we follow DARTS's protocol: we run \our $4$ times with different random seeds and pick the best architecture based on its validation performance. We then randomly reinitialize the weights and retrain for $600$ epochs. During search we use half of the training set as validation. %We repeat the full training of the best architecture $4$ times and report mean and standard deviation for a fair comparison with other approaches.
To fairly compare with more recent methods, we also re-train the best searched architecture using AutoAugment and Extended Training \cite{Cubuk_AutoAugment}.

\paragraph{Results.}
Both \our implementations perform well on this dataset (Table~\ref{table:Cifarresults}). 
Our algorithm is designed to perform comparably to \cite{Liu2019_DARTS} but with an order of magnitude less memory. However, \our actually achieves higher accuracy. The reason for this is that DARTS is forced to search for an $8$ cell architecture and subsequently stack the same cells $20$ times; \our, on the other hand, can directly search on the final number of cells leading to better results. We also report our results when using only $8$ cells: even though the network is much smaller, it still performs competitively with 1st-order $20$-cell DARTS. This is explored in more depth in Section~\ref{sec:alt_expers}. In terms of memory usage with a batch size of 1, MANAS $8$ cells required only 1GB of GPU memory, while DARTSv1 utilized more than 8.5GB and DARTSv2 required 9.6GB, making both versions of DARTS unpractical to work with datasets with larger image sizes.

\cite{Cai2018_proxylessNAS} is another method designed as an efficient alternative to DARTS; unfortunately the authors decided to a) use a different search space (PyramidNet backbone; \cite{Han2017_pyramidnet}) and b) offer no comparison to random sampling in the given search space. For these reasons we feel a numerical comparison to be unfair. Furthermore our algorithm uses half the GPU memory (they sample $2$ paths at a time) and does not require the reward to be differentiable.
Lastly, we observe similar gains when training the best \our/\our-LS architectures with an extended protocol (AutoAugment + 1500 Epochs + 50 Channels, in addition to the DARTS protocol).



\subsection{Results on ImageNet}


\begin{table}[t]
\caption{Comparison with state-of-the-art image classifiers on ImageNet (mobile setting). The four row blocks represent: human-designed, NAS, MANAS search with DARTS training protocol and best searched MANAS retrained with extended protocol (AutoAugment + 600 Epochs + 60 Channels).}
  \label{table:ImageNetresults}
\centering
  \resizebox{\textwidth}{!}{
\begin{tabular}{p{6cm}p{1.5cm}p{1cm}p{1.8cm}p{1.5cm}llllllll}
    \toprule
    %\cmidrule(r){1-2}
    Architecture   & Test Error (\%) & Params (M) & Search Cost (GPU days) & Search Method\\
    \midrule
    %Inception-v1 \cite{Szegedy2017_inception} & $30.2$ & $6.6$ & & manual \\
    %MobileNet \cite{Howard2017_MobileNets} & $29.4$ & $4.2$ & & manual \\
    %ShuffleNet 2x (v1) \cite{Ma2018_ShuffleNetV1} & $29.1$ & ~$5$ & & manual \\
    ShuffleNet 2x (v2)  \cite{Zhang2018_ShuffleNetV2} & $26.3$ & ~$5$ & --- & manual \\
    \midrule
    NASNet-A \cite{Zoph2018_NASNet} & $26.0$ & $5.3$ & $1800$ & RL \\
    %NASNet-B \cite{Zoph2018_NASNet} & $27.2$ & $5.3$ & $1800$ & RL \\
    %NASNet-C \cite{Zoph2018_NASNet} & $27.5$ & $4.9$ & $1800$ & RL \\
    %AmoebaNet-A \cite{Real2018_AmoebaNet} & $25.5$ & $5.1$ & $3150$ & evolution \\
    %AmoebaNet-B \cite{Real2018_AmoebaNet} & $26.0$ & $5.3$ & $3150$ & evolution \\
    AmoebatNet-C \cite{Real2018_AmoebaNet} & $24.3$ & $6.4$ & $3150$ & evolution \\
    PNAS \cite{Liu2018_PNAS} & $25.8$ & $5.1$ & $225$ & SMBO \\
    SNAS \cite{Xie19_SNAS} (search on C10) & $27.3$ & $4.3$ & $1.5$ & gradient \\
    DARTS \cite{Liu2019_DARTS} (search on C10) & $26.7$ & $4.7$ & $4$ & gradient      \\
    %EfficientNet B0 \cite{tan2019efficientnet} & $23.7$ & $5.3$ & $~3000$ & RL \\ %not in darts search space
    GDAS \cite{DBLP:conf/cvpr/DongY19} (search on C10) & $27.5$ & $4.4$ & $0.17$ & gradient \\
    EffPNet \cite{wang2021surrogate} (search on C10) & $27.1$ & $-$ & $3$ & evolution \\
    NASP \cite{DBLP:conf/aaai/YaoXTZ20} (search on C10) & $26.3$ & $9.5$ & $0.2$ & proximal \\

    

    \midrule
    Random sampling & $27.75$ & $2.5$ & --- & --- \\ 
    \our (search on C10) & $26.47$ & $2.6$ & $2.8$ & MA \\ 
    \our (search on IN) & $26.15$ & $2.6$ & $110$ & MA \\
    \midrule
    \our (search on C10) + AutoAugment & 26.81 & $2.6$ & --- & MA \\ 
    \our (search on IN) + AutoAugment & 25.26 & $2.6$ & --- & MA \\
    \bottomrule
  \end{tabular}
  }
\end{table}





\paragraph{Evaluation. }
To evaluate the results on ImageNet we train the final architecture for $250$ epochs. We report the result of the best architecture out of $4$, as chosen on the validation set for a fair comparison with competing methods.
As search and augmentation are very expensive we use only \our and not \our-LS, as the former is computationally cheaper and performs slightly better on average.
%\Blue{We also re-train the best searched architecture using AutoAugment \cite{Cubuk_AutoAugment} and } \Red{$???$ epochs.}


\paragraph{Results. }
We provide results for networks searched both on CIFAR-10 and directly on ImageNet, which is made possible by the computational efficiency of \our (Table~\ref{table:ImageNetresults}). 
When compared to SNAS, DARTS, GDAS and other methods, using the same search space, \our achieves state-of-the-art results both with architectures searched directly on ImageNet %($0.85$ p.p. improvement) 
and also with architectures transferred from CIFAR-10. %($0.55$ p.p. improvement).
We observe similar improvements when training the best \our architecture with an extended training protocol (AutoAugment + 600 Epochs + 60 Channels, in addition to the DARTS protocol), resulting in a final test error of 25.26\% when directly searching on ImageNet.




\subsection{Results on new datasets: Sport-8, Caltech-101, MIT-67}
\label{sec:alt_expers}

\paragraph{Evaluation. }
The idea behind NAS is that of finding the optimal architecture, given \textit{any} sets of data and labels. Limiting the evaluation of current methods to CIFAR-10 and ImageNet could potentially lead to algorithmic overfitting. Indeed, recent results suggest that the search space was engineered in a way that makes it very hard to find a a bad architecture \cite{Li2019_random,Sciuto2019_random,Yang2020NASEFH,wan2022on}. To mitigate this, we propose testing NAS algorithms on $3$ datasets (composed of regular sized images)
%, which are composed of images larger than those of CIFAR-10 and
that were never before used in this setting, but have been historically used in the CV field: 
Sport-8, Caltech-101 and MIT-67, described briefly in the Appendix. 
For these set of experiments we run the algorithm $8$ times and report mean and std. We perform this both for $8$ and $14$ cells; we do the same with DARTS (which, due to memory constraints can only search for $8$ cells).
As baselines, we consider random search and random sampling.
For the latter we simply sample uniformly $8$ architectures from the search space. To efficiently implement random search, we follow \cite{Li2019_random} and perform experiments on random search with WS.
Each proposed architecture is trained from scratch for $600$ epochs as in the previous section.

\paragraph{Results.} 
\our manages to outperform the random baselines and significantly outperform DARTS, especially on $14$ cells (Figure \ref{fig:ablation_1}): this clearly shows that the optimal cell architecture for $8$ cells is \textit{not} the optimal one for $14$ cells. 


\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{manas_8.pdf}
    \includegraphics[width=0.49\textwidth]{manas_14.pdf}
    \vspace{2pt}
    \caption{Comparing \our, random sampling, random search with WS \cite{Li2019_random} and DARTS \cite{Liu2019_DARTS} on $8$ and $14$ cells. Average results of $8$ runs. Note that DARTS was only optimised for $8$ cells due to memory constraints.}
    \label{fig:ablation_1}
\end{figure}


%\R{A number of limitations exist in each of these approaches. \cite{Sciuto2019_random} show that, on average, a random architecture outperforms those obtained by NAS methods, mainly due to the limited search space used.
%\cite{Sciuto2019_random} further show that the ranking of architectures provided by NAS methods does not reflect their true ranking in terms of performance, and link the cause of this to the weight sharing property.
%Similarly, performance predictors need to be well tuned in order to avoid this ranking distortion problem.
%\cite{2019arXiv190400438A} investigate the interpretability of ENAS (\cite{Pham2018_ENAS}) and show that the controller does not learn to encode past actions, hence does not learn anything meaningful.
%Additionally, the cell-stacking approach used in DARTS---where only two different cells are learned and stacked sequentially to achieve a pre-selected depth---is widely used for computational efficiency, although it represents a strong restriction on the structure of the network.}

%\R{We provide further results that reveal the importance of network depth. Essentially, random baseline architectures in deep network spaces are capable of learning easily regardless of the operations available, thus masking the intrinsic capabilities of the search methods.}





%\begin{table}[t]
%  \caption{Comparison with Random Architectures and DARTS on 3 datasets}
%  \label{AblationTable}
%  \centering
%  \begin{tabular}{p{3.8cm}P{2.4cm}P{2.4cm}P{2.4cm}lllllllllllllll}
%    \toprule
%    \textbf{Architecture} &
%    \multicolumn{3}{c}{\textbf{Test error ($\%$)}} \\
%    \midrule
%    %& \multicolumn{3}{c}{Search Cost (GPU days)} \\
%    & \textbf{Sport-8} & \textbf{Caltech-101} & \textbf{MIT-67} \\
%    % & Sport & Caltech & MIT \\
%    %\midrule
%    DARTS \cite{Liu2019_DARTS} & $8.28$ & $14.54$ & $31.01$ 
%    %& $0.1$* & $0.1$* & $0.2$* 
%    \\
%    %\midrule
%    Random & $5.85$ & $13.64$ & $29.35$ 
%    %& & & 
%    \\
%    %\midrule
%    \our & $5.53$ & $13.43$ & $29.21$ 
%    %& $0.007$ & $0.03$ & $0.05$
%    \\ 
%    \bottomrule
%  \end{tabular}
%\%end{table}


\begin{table}[t]
    \caption{Results of \our with complexity constraints using different penalty ($\lambda$) values on CIFAR-10.\label{tab:constraints}}
    \centering
      \resizebox{0.55\textwidth}{!}{
        %\begin{tabular}{p{7.2cm}p{1.5cm}p{1cm}p{1.8cm}p{1.5cm}}
      \begin{tabular}{lll} 
      \toprule
     $\lambda$ & Test Error (\%) & Inference Time (ms)                 \\ \midrule
     $0$ & $2.91$ & $1.255$ $\pm$ $0.012$ \\
     $0.1$ & $3.12$ & $1.196$ $\pm$ $0.009$ \\
     %$0.20$ & $2.58$ & $1.177$ $\pm$ $0.006$ \\
     $0.25$ & $2.94$ & $1.190$ $\pm$ $0.008$ \\
     %$0.3$ & $2.89$ & $1.167$ $\pm$ $0.007$ \\
     %$0.4$ & $2.89$ & $1.136$ $\pm$ $0.006$ \\
     $0.5$ & $3.04$ & $1.183$ $\pm$ $0.006$ \\
     %$0.6$ & $2.67$ & $1.131$ $\pm$ $0.003$ \\
     %$0.7$ & $2.90$ & $1.170$ $\pm$ $0.005$ \\
     $0.75$ & $2.54$ & $1.179$ $\pm$ $0.005$ \\
     %0.8 -> running
     %$0.9$ & $2.76$ & $1.157$ $\pm$ $0.009$ \\
     $1$ & $2.69$ & $1.164$ $\pm$ $0.006$ \\ \bottomrule               
    \end{tabular}
  }
\end{table}

\subsection{Results with Complexity Constraint}
\label{sec:complexity_constraint}

\paragraph{Evaluation. }
To evaluate the results of \our in a complexity constraint setting, we eadded the inference time of the generated architectures as a complexity constraint to the training. For this, we update the training loss with the constraint of the inference time that the generated architecture takes to classify an image: $\loss^{(\text{train})}_t(\bm{a}_t) =\loss^{(\text{train})}_t(\archi_t,\bm{w}_t )+\lambda L_t(\archi_t,\bm{w}_t )$, where $L_t$ is the inference time to classify one image, and $\lambda$ defines the importance given to $L_t$. 
Here, the $\lambda$ serves the purpose of varying the importance given to the inference time whilst searching. By increasing $\lambda$, the inference time constraint has a higher importance.

%we train the final architecture for $250$ epochs. We report the result of the best architecture out of $4$, as chosen on the validation set for a fair comparison with competing methods.
%As search and augmentation are very expensive we use only \our and not \our-LS, as the former is computationally cheaper and performs slightly better on average.
\paragraph{Results.} 
We evaluate \our with different $\lambda$ values using a single GPU (Table \ref{tab:constraints}), and observe that 
%\our can be easily trained with latency constraints by updating the training loss. 
by increasing the importance given to the inference, \our consistently generates architectures with a lower inference time, with similar accuracies. This experiment shows that \our can be extended for searching with multiple objectives, by modifying the training loss.%, meaning that it is capable of converging to `very good' minima even with added complexity.


%We evaluate \our with complexity constraints by using the inference time of the generated architectures as a constraint to \our training. For this, we update the training loss with the constraint of the inference time that the generated architecture takes to classify an image: $\loss^{(\text{train})}_t(\bm{a}_t) =\loss^{(\text{train})}_t(\archi_t,\bm{w}_t )+\lambda L_t(\archi_t,\bm{w}_t )$, where $L_t$ is the inference time to classify one image, and $\lambda$ defines the importance given to $L_t$. 
%By varying the lambda, the importance of the inference varies.
%, as it influences more or less the adjustment of the weights when back-propagating the loss. 
%We evaluate \our with different $\lambda$ values using a single 1080Ti GPU (Table \ref{tab:constraints}), and observe that 
%\our can be easily trained with latency constraints by updating the training loss. 
%by increasing the importance given to the inference, \our consistently generates architectures with a lower inference time, with similar accuracies.%, meaning that it is capable of converging to `very good' minima even with added complexity.


==> MANAS Machine Learning Journal/intro.tex <==

Determining an optimal architecture is key to accurate deep neural networks (DNNs) with good generalisation properties \cite{Szegedy2017_inception,Huang2017_densenet,He2016_resnet,Han2017_pyramidnet,Conneau2017_VDLCNN,Merity2018_LSTM}. Neural architecture search (NAS), which has been formulated as a graph search problem, can potentially reduce the need for application-specific expert designers allowing for a wide-adoption of sophisticated networks in various industries. \cite{ZophLe17_NAS} presented the first modern algorithm automating structure design, and showed that resulting architectures can indeed outperform human-designed state-of-the-art convolutional networks \cite{Ko2019,Liu2019_DARTS}. 
However, even in the current settings where flexibility is limited by expertly-designed search spaces, NAS problems are computationally very intensive with early methods requiring hundreds or thousands of GPU-days to discover state-of-the-art architectures \cite{ZophLe17_NAS,Real2017_EvoNAS,Liu2018_PNAS,Liu18_HEVO}.


%For training deep neural networks (DNNs), it becomes crucially important to find the optimal architecture  \cite{Szegedy2017_inception,Huang2017_densenet,He2016_resnet,Han2017_pyramidnet,Conneau2017_VDLCNN,Merity2018_LSTM}.
%Unfortunately, this requires an iterative process of trial and error, which is a time consuming procedure even for the most expert practitioners.
%In 2017 the first modern approach to this iterative process was proposed: Neural Architecture Search (NAS; \cite{ZophLe17_NAS}) aims to automate the design of DNNs and has showed promising results by outperforming human-designed, state-of-the-art architectures for convolutional and recurrent networks \cite{Ko2019,Liu2019_DARTS}.

%In image classification, for instance, the NAS problem is to search for the best combination of convolutional filters, pooling operations and fully connected layers in a Convolutional Neural Network (CNN) in order to maximise the network's predictive accuracy.

%However, even with the restrictive search spaces currently used, NAS is highly computationally intensive, the earliest methods requiring hundreds or thousands of GPU-days to discover state-of-the-art architectures \cite{ZophLe17_NAS,Real2017_EvoNAS,Zoph2018_NASNet,Real2018_AmoebaNet,Liu2018_PNAS,Liu18_HEVO}.

Researchers have used a wealth of techniques ranging from reinforcement learning, where a controller network is trained to sample promising architectures~\cite{ZophLe17_NAS,Zoph2018_NASNet,Pham2018_ENAS,bender2020can}, to evolutionary algorithms that evolve a population of networks for optimal DNN design~\cite{Real2018_AmoebaNet,Liu18_HEVO,lopes2022towards}, to optimization on random graphs \cite{ru2020nago}. Alas, these approaches are inefficient and can be extremely computationally and/or memory intensive as some require all tested architectures to be trained from scratch.
Weight-sharing, introduced in ENAS~\cite{Pham2018_ENAS}, can alleviate this problem.
%training all sampled architectures from scratch can be remedied through weight-sharing as introduced in ENAS~\cite{Pham2018_ENAS}. 
Even so, these techniques cannot easily scale to large datasets, e.g., ImageNet, relying on human-defined heuristics for architecture transfer.
Recently, low-fidelity estimates, performance predictors and guiding mechanisms have also been studied to improve the search cost and reduce the memory and computation required \cite{mellor2021neural,lopes2021epe,white2021bananas,ning2021evaluating,white2021powerful,lopes2022guided}. More, gradient-based frameworks enabled efficient solutions by introducing a continuous relaxation of the search space. For example, DARTS \cite{Liu2019_DARTS} uses this relaxation to optimise architecture parameters using gradient descent in a bi-level optimisation problem, while SNAS \cite{Xie19_SNAS} updates architecture parameters and network weights under one generic loss.
Still, due to memory constraints the search has to be performed on $8$ cells, which are then stacked $20$ times for the final architecture. 
%These results were further improved by ProxylessNAS and SNAS~\cite{Cai2018_proxylessNAS}.  Due to the combinatorial explosion in the search space, algorithms from the gradient-based family have to approximate NAS by learning a fixed 
%approximate NAS by searching over building-block components (cells), which are then stacked together to form the deep network. 
This solution is a coarse approximation to the original problem as shown in Section~\ref{sec:exp} 
of this work and in \cite{Yang2020NASEFH,Sciuto2019_random,Li2019_random}, receiving some criticisms outlined in \cite{Zela2020Understanding,Yang2020NASEFH,wan2022redundancy}.
In fact, we show that searching directly over 20 cells leads to a reduction in test error (8\% relative to~\cite{Liu2019_DARTS}).
ProxylessNAS \cite{Cai2018_proxylessNAS} is one exception, as it can search for the final models directly; nonetheless they still require twice the amount of memory used by our proposed algorithm, while offering no theoretical guarantees.

To enable the possibility of large-scale joint optimisation of deep architectures we contribute MANAS, the first multi-agent learning algorithm for neural architecture search.
Our algorithm combines the memory and computational efficiency of multi-agent systems, which is achieved through action coordination with the theoretical rigour of online machine learning, allowing us to balance exploration versus exploitation optimally. % between network structures. 
Due to its distributed nature, MANAS enables large-scale optimisation of deeper networks while learning different operations per cell. Theoretically, we demonstrate that MANAS implicitly coordinates learners to recover vanishing regrets, guaranteeing convergence.
Empirically, we show that our method achieves state-of-the-art accuracy results among methods using the same evaluation protocol but with significant reductions in memory (1/8th of \cite{Liu2019_DARTS}) and search time (70\% of \cite{Liu2019_DARTS}).

The multi-agent (MA) framework is inherently scalable and allows us to tackle an optimization problem that would be extremely challenging to solve efficiently otherwise: the search space of a single cell is $8^{14}$ and there is no fast way of learning the joint distribution, as needed by a single controller. More cells to learn exacerbates the problem, and this is why MA is required, as for each agent the size of the search space is always constant.

In short, our contributions can be summarised as: 
(1) framing NAS as a multi-agent learning problem (MANAS) where each agent supervises a subset of the network; agents coordinate through a credit assignment technique which infers the quality of each operation in the network, without suffering from the combinatorial explosion of potential solutions.  
(2) Proposing two lightweight implementations of our framework that are theoretically grounded. The algorithms are computationally and memory efficient, and achieve state-of-the-art results on CIFAR-10 and ImageNet when compared with competing methods. Furthermore, \our allows search \textit{directly} on large datasets (e.g. ImageNet).
(3) Presenting $3$ news datasets for NAS evaluation to minimise algorithmic overfitting; offering a fair comparison with the often ignored random search \cite{Li2019_random} and random sampling \cite{Yang2020NASEFH,Sciuto2019_random} baselines; and presenting a complexity constraint analysis of \our.

%Despite the good empirical results, recent works have questioned the efficacy of current NAS methods, specifically their small gains over random architectures, seemingly a consequence of their very well engineered search spaces and the weight-sharing assumption \cite{Sciuto2019_random,Li2019_random}.
%Based on these observations, we show that it is possible to find competitive architectures with a much smaller computational budget than competing methods.




%introduced a continuous relaxation of the search space to optimise for 

%\textit{Gradient} approaches use a continuous relaxation on the search space.
%DARTS \cite{Liu2019_DARTS} uses this relaxation to optimise the architecture parameters using gradient descent in a bi-level optimisation problem. 


%This removes the need for controllers, hypernetworks or performance predictors, but due to computational constraints the search is for network components (\textit{cells}) which are stacked, as opposed to global network architecture.
%ProxylessNAS \cite{Cai2018_proxylessNAS} improves the efficiency of DARTS by activating only 2 out of 8 possible paths per edge during the search phase; and SNAS \cite{Xie19_SNAS} puts architecture parameters and network weights under one generic loss.
%We note that all these GD-based approaches use the weight-sharing assumption introduced by ENAS.


%For instance, NAS and NASNet adopt a controller network for sampling promising architectures by using validation accuracy as rewards. 


%have focused on computationally-efficient methods \cite{Pham2018_ENAS,Liu2019_DARTS,Cai2018_proxylessNAS} but most still do not scale well to large image datasets such as ImageNet.
%In practice, architecture search is almost always performed on smaller \textit{proxy} datasets such as CIFAR-10 (to our knowledge, the only exception is ProxylessNAS \cite{Cai2018_proxylessNAS}), and the best searched architecture then transferred to large datasets.

%There are a few different fundamental approaches to NAS.
%\textit{Reinforcement Learning} approaches use a controller network that learns to sample promising architectures in a guided fashion by using the validation accuracy as the reward.
%NAS and NASNet \cite{ZophLe17_NAS,Zoph2018_NASNet} are extremely computationally-intensive as they require all tested architectures to be trained from scratch.
%To avoid this, ENAS \cite{Pham2018_ENAS} introduced the assumption of \emph{weight sharing}---where network weights are shared by all tested architectures.
%A number of works search progressively (i.e., in order of increasing complexity): 
%EAS \cite{Cai2018_LayerEAS,Cai2018_PathEAS} uses layer-level and path-level function-preserving transformations;
%PNAS \cite{Liu2018_PNAS} learns a performance predictor to guide architecture proposals;
%and SMASH \cite{Brock2018_SMASH} learns a hypernetwork to dynamically generate shared network weights.
%\textit{Evolutionary} approaches evolve a population of architectures through biologically-inpired processes (death, reproduction, mutation) in order to find good architectures.
%AmoebaNet \cite{Real2018_AmoebaNet} evolves networks in the NAS search space and HierarchicalEvo \cite{Real2018_AmoebaNet} uses a new hierarchical representation imitating a modularised design.
%\textit{Gradient} approaches use a continuous relaxation on the search space.
%DARTS \cite{Liu2019_DARTS} uses this relaxation to optimise the architecture parameters using gradient descent in a bi-level optimisation problem. This removes the need for controllers, hypernetworks or performance predictors, but due to computational constraints the search is for network components (\textit{cells}) which are stacked, as opposed to global network architecture.
%ProxylessNAS \cite{Cai2018_proxylessNAS} improves the efficiency of DARTS by activating only 2 out of 8 possible paths per edge during the search phase; and SNAS \cite{Xie19_SNAS} puts architecture parameters and network weights under one generic loss.
%We note that all these GD-based approaches use the weight-sharing assumption introduced by ENAS.

%Despite the good empirical results, recent works have questioned the efficacy of current NAS methods, specifically their small gains over random architectures, seemingly a consequence of their very well engineered search spaces and the weight-sharing assumption \cite{Sciuto2019_random,Li2019_random}.
%Based on these observations, we show that it is possible to find competitive architectures with a much smaller computational budget than competing methods.

%Currently, gradient methods using weight-sharing and the search space originally proposed by DARTS achieve the best trade-off between accuracy and computational efficiency.
%Our approach follows DARTS, but addresses two significant limitations:
%first, our method uses only 1/8th of the memory required by DARTS and, therefore, allows \textit{search} to be performed on deeper networks;
%second, our method is able to learn different operations in each cell, as opposed to learning only two different types of cells as in DARTS.


%The first and main contribution of this paper is to propose methods that simultaneously are computationally efficient, memory efficient, theoretically grounded and that recover state of the arts results of more heavy approaches.
%To obtain such a result we \textbf{1)}  frame NAS as a multi-agent learning problem where each agent is in charge of the architecture of a subset of the network,  \textbf{2)} we propose two extremely lightweight implementations of our framework that implement weight sharing and spare architecture search, \textbf{3)}
%our agents are implicitly coordinated through an a credit assignment technique that infers the quality of each operation in the network without suffering from the combinatorial explosion of potential solutions.
%When evaluating empirically our proposed methods, we propose $3$ new datasets for a more unbiased evaluation. Our results show that we either recover or beat the state of the art  while using less memory. This allow for architecture search directly on large datasets such as ImageNet.
 %We also discuss some of the problems with the current approaches to NAS.




%Our solution is to frame NAS as a problem of cooperative multi-agent learning in which each agent must locally pick the best operation out of the available ones.

%As a step towards true NAS, in section X we expand the search space by including new operations that, while not immediately contributing towards an increase in state of the art, help us better evaluate our and competing methods against the baseline of random search.


% AND we propose a larger search space to better evaluate the different methods


% \R{The contributions of this paper are multiple: 1) we frame NAS as a problem of multiagent learning; 2) we propose two extremely lightweight implementations of our framework;  3) we propose $3$ new datasets for a more unbiased evaluation; and 4) we \R{highlight} some of the problems with the current approaches to NAS}
% % AND we propose a larger search space to better evaluate the different methods

% \R{In this paper we propose a multi-agent reinforcement learning approach to NAS that (i) achieves state-of-the-art results; (ii) has low computational search cost, thus allowing for architecture search directly on large datasets such as ImageNet.}


%Our main contributions are two-fold:\\\\
%(i) Reduced memory consumption, which enables direct search on a given number of stackings and/or on larger data inputs. \\\\
%(ii) A novel approach to sampling and updating the architecture weights, which is yields faster training time and is theoretically sound (???)

%Current approaches to NAS fall into three broad categories:
%those using reinforcement learning train a controller network to sample new architectures (\R{REFS})
%\R{[a sentence about the dominant cell-structure approach in the literature]}




==> MANAS Machine Learning Journal/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> MANAS Machine Learning Journal/notations.tex <==
% \newtheorem{remark}{Remark}

\newcommand{\setArmsmo}{\{1,\ldots,K\}}
\newcommand{\estCumulGainVector}{\bm{\widetilde B} }
\newcommand{\cumulGain}{\bm{ B} }
\newcommand{\gap}{\Delta}

\newcommand{\nArms}{K}

\newcommand{\estGainVector}{\bm{ \tilde \beta}}
\newcommand{\gainVector}{\bm{\beta}}
\newcommand{ \var}{\sigma}




\newcommand{\timeHorizon}{T }
\newcommand{\Pro}{P}

\newcommand{\agent}{\mathcal{A}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\imporEst}{\tilde \bm{l}}

\newcommand{\opWeights}{\bm{w}}

\newcommand{\archi}{\mathcal{Z}}
\newcommand{\recomArchi}{A}

\newcommand{\Real}{\mathbb{R}}
\newcommand{\batch}{B}

%\definecolor{autoblue}{RGB}{1, 76, 103}

%\definecolor{autored}{RGB}{ 168, 23, 11}

%\definecolor{autogreen}{RGB}{92, 104, 20}


==> MANAS Machine Learning Journal/related.tex <==

\section{Related work}



\our derives its search space from DARTS \cite{Liu2019_DARTS} and is therefore most related to other gradient-based NAS methods that use the same search space.
SNAS \cite{Xie19_SNAS} appears similar at a high level, but has important differences: 1) it uses GD to learn the architecture parameters. This requires a differentiable objective (MANAS does not) and leads to 2) having to forward all operations (see their Eqs.5,6), thus negating any memory advantages (which MANAS has), and effectively requiring repeated cells and preventing search on ImageNet. Sequent gradient-base proposals improve upon baselines by introducing regularization mechanisms to improve the final performance of the generated architectures \cite{Zela2020Understanding,DBLP:conf/icml/ChenH20,DBLP:conf/iclr/ChuW0LWY21}, whilst still suffering from the aforementioned problems.

ENAS \cite{Pham2018_ENAS} is also very different: its use of RL implies dependence on past states (the previous operations in the cell). It explores not only the stochastic reward function but also the relationship between states, which is where most of the complexity lies.
Furthermore, RL has to balance exploration and exploitation by relying on sub-optimal heuristics, while MANAS, due to its theoretically optimal approach from online learning, is more sample efficient.
Finally, ENAS uses a single LSTM (which adds complexity and problems such as exploding/vanishing gradients) to control the entire process, and is thus following a monolithic approach.
Indeed, at a high level, our multi-agent framework can be seen as a way of decomposing the monolithic controller into a set of simpler, independent sub-policies. This provides a more scalable and memory efficient approach that leads to higher accuracy, as confirmed by our experiments.

